More Than Positive and Negative: Communicating Fine Granularity in Medical Diagnosis

With the advance of deep learning, much progress has been made in building powerful artificial intelligence (AI) systems for automatic Chest X-ray (CXR) analysis. Most existing AI models are trained to be a binary classifier with the aim of distinguishing positive and negative cases. However, a large gap exists between the simple binary setting and complicated real-world medical scenarios. In this work, we reinvestigate the problem of automatic radiology diagnosis. We first observe that there is considerable diversity among cases within the positive class, which means simply classifying them as positive loses many important details. This motivates us to build AI models that can communicate fine-grained knowledge from medical images like human experts. To this end, we first propose a new benchmark on fine granularity learning from medical images. Specifically, we devise a division rule based on medical knowledge to divide positive cases into two subcategories, namely atypical positive and typical positive. Then, we propose a new metric termed AUC$^\text{FG}$ on the two subcategories for evaluation of the ability to separate them apart. With the proposed benchmark, we encourage the community to develop AI diagnosis systems that could better learn fine granularity from medical images. Last, we propose a simple risk modulation approach to this problem by only using coarse labels in training. Empirical results show that despite its simplicity, the proposed method achieves superior performance and thus serves as a strong baseline.

==> sec/exp_v0.tex <==
\section{Experiments}
\label{sec:exp}

\subsection{Data}
We evaluate our method on the large-scale CXR dataset MIMIC-CXR-JPG~\cite{johnson2019mimicjpg}. MIMIC-CXR-JPG is wholly derived from MIMIC-CXR~\cite{johnson2019mimic}, which consists of JPG format files converted from the original DICOM images. Officially, the MIMIC-CXR-JPG dataset is organized into a training set of 222,758 studies from 64,586 patients, a validation set of 1808 studies from 500 patients, and a test set of 3269 studies from 293 patients. Each study consists of a medical report and one or more Chest X-rays. In this work, we only consider radiographs with anteroposterior or posteroanterior views.

The labels we use are proposed by Zhang et al. (2023)~\cite{zhang2023expert}. The authors extract from reports multiple levels of disease severity, as well as traditional categories of negative, uncertain, and positive. In addition to that, we further extract keywords on change in time such as ``improve'' and ``worsen'', using the same extraction tool as in~\cite{zhang2023expert}. The multiple severity levels and keywords on change in time jointly compose the fine-grained positive labels used in this work. Note that the fine-grained labels are only used in validation. We build a metric upon the fine-grained positive labels for evaluation of fine granularity learning. Details of the metric are elaborated in Sec.~\ref{sec:metric}.
% Officially, the MIMIC-CXR-JPG dataset is organized into a training set of 368,960 images from 64,586 patients, a validation set of 2991 images from 500 patients, and a test set of 5159 images from 293 patients. 

% Given that there are few uncertain samples \pxy{(TODO: how many?)} in the official validation and the test set, we split the training set into 5 folds among which 4 folds are used for training and 1 fold is held out for validation. Note that we make the split based on individual patients so that no images from the same patient are used in both training and validation. 

\subsection{Evaluation Metrics} \label{sec:metric}

Most previous works use the area under the receiver operating characteristic curve (AUC) of positive and negative samples as the metric~\cite{irvin2019chexpert, yuan2021large, pham2021interpreting} for radiology diagnosis. Although it encourages an AI system to distinguish positive and negative samples, it is incapable of evaluating complicated cases within a single class.

In this work, we propose a new benchmark for fine granularity learning with coarsely annotated medical images, termed AUC$^{\text{FG}}$. We first devise a division rule to group fine-grained positive labels into two categories, namely atypical positive and typical positive. Then, we calculate the AUC between these two categories, with atypical positive being 0 and typical positive being 1. The details of the division rule are presented in Tab.~\ref{tab:atypical}. Specifically, we make the division based on two dimensions, which are severity and change in time. On the one hand, for severity, slight symptoms are classified as atypical positive (\eg, ``small", ``minor'', ``mild''), while significant symptoms are grouped as typical positive (\eg, ``severe'', ``acute''). On the other hand, change to a better condition is considered atypical positive (\eg, ``improve'', ``decrease''), while change to a worse condition is considered typical positive (\eg, ``worsen'', ``increase''). If a sample has no fine-grained labels, it is treated as typical positive (\eg, ``There is consolidation in the right lung.''). We confirm the rationality of the division rule with human experts.

With the proposed metric, we are able to evaluate how well a model can discover the fine-granularity knowledge in medical images. A higher AUC$^{\text{FG}}$ indicates a better ability to distinguish atypical and typical positive and a better alignment with human expert evaluation.



\subsection{Experimental Setup}
\paragraph{Training.}
We use the official split of MIMIC-CXR-JPG for training and validation. For all experiments in this work, we use the same backbone network and training process for fair comparison. We choose DenseNet121~\cite{huang2017densely} as the backbone network, following the CheXpert paper~\cite{irvin2019chexpert}. The backbone network is initialized with ImageNet pre-trained weights\footnote{We use the official pre-trained weights provided by PyTorch. See \url{https://pytorch.org/vision/0.10/_modules/torchvision/models/densenet.html}.} for faster convergence except for the last fully connected layer which is randomly initialized. The input images are rescaled to $224 \times 224$ pixels. We use the Adam~\cite{kingma2014adam} optimizer for training with $\beta$-parameters of $\beta_1 = 0.9$, $\beta_2 = 0.999$, a fixed learning rate of $1e^{-4}$ and a weight decay of $0$. The model is trained for 50,000 iterations with a total batch size of 32 on 2 GPUs. In this way, all experiments have the same amount of training. We save checkpoints every 10,000 iterations, obtaining 5 checkpoints in each run.

\input{tables/main_res}
\paragraph{Validation.}
For each method, we run the model three times, each with a different seed. We choose the best checkpoint on the validation set from each run and report the mean and standard deviation of the three best checkpoints. We validate our method on consolidation and edema individually, two pathologies of clinical importance and prevalence. Note that only samples with positive labels are involved in validation since our goal is to learn fine-grained knowledge within the positive class. 

\subsection{Main Results}
We compare our method to several baseline uncertainty approaches under the proposed metric AUC$^{\text{FG}}$ in Tab.~\ref{tab:main_res}. The baseline uncertainty approaches are trained with the CE loss by default if not otherwise specified. We report mean $\pm$ std of three best checkpoints on the validation set for each method. One can see that U-Ones achieves the best performance among the three baseline approaches. For edema, U-Ignore is almost as good as U-Ones but U-Zeros leads to a significant drop in performance. This is probably because most uncertain phrases for edema actually convey findings that are more positive such as ``likely superimposed pulmonary edema.'' However, such a contrast is not observed for consolidation. Both U-Zeros and U-Ones achieve higher performance than U-Ignore for consolidation, which indicates the information in uncertain consolidation samples is beneficial to learning fine-grained knowledge.

% However, for consolidation, there are more negative-like uncertain expressions like ``an underlying consolidation is not excluded.'' This could be an explanation of U-Zeros better than U-Ignore for consolidation. 
 
Finally, our method outperforms all the baseline approaches by a large margin.
% ($\ge$ 0.02 absolute improvement) 
It achieves AUC$^{\text{FG}}$ of 0.8038 for consolidation, which is more than 0.03 higher than U-Ones, and 0.6663 for Edema, which is more than 0.02 higher than U-Ones.
This demonstrates the effectiveness of risk modulation for learning fine granularity without fine-grained labels. We conduct ablation studies in Sec.\ref{sec:abl} to study the effect of applying risk modulation on positive and uncertain cases individually.

% , regardless of the tendency of uncertain samples. 

% This demonstrates that our method has a strong capability of communicating fine granularity among all samples of the positive label.

% an effective learning of fine-grained knowledge.

\subsection{Ablation Studies} \label{sec:abl}
% \subsubsection{Hyper-parameter}
\paragraph{Hyper-parameter $\tau$.} We show in Fig.~\ref{fig:tau} the results of varing $\tau$ in Eq.~\ref{eq:pce}. The line and the band represent the mean and the standard deviation respectively. For both consolidation and edema, our method outperforms the baseline method in a wide range of $\tau$ (from 0.3 to 0.5 for consolidation, from 0.2 to 0.5 for edema), while the std of our method is lower or on par with the baseline. This shows the robustness of our method towards the hyper-parameter.

\paragraph{Effect on Individual Classes.} We study the effect of applying the risk modulation loss on each individual class, \ie, the uncertain and the positive class. The results are shown in Tab.~\ref{tab:abl_pu}. One can see that for both consolidation and edema, applying the risk modulation loss only on positive samples achieves better results than the baseline when uncertain samples are ignored. This shows the effectiveness of risk modulation for learning fine-grained knowledge from positive samples. When the risk modulation is applied to uncertain samples in addition to positive samples, the performances are further improved, which demonstrates that U-RM can serve as an effective uncertainty approach.

\input{tables/abl_pu}

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/tau_con.pdf}
        \caption{Caption}
        \label{fig:tau_con}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{\linewidth}
        \centering
        \includegraphics[width=\linewidth]{figures/tau_ede.pdf}
        \caption{Caption}
        \label{fig:tau_ede}
    \end{subfigure}
    \caption{Caption}
    \label{fig:tau}
\end{figure}


\input{tables/atypical2}
% \input{tables/main_res_old}


==> sec/intro_old.tex <==
\section{Introduction}
\label{sec:intro}

Medical artificial intelligence (AI) has demonstrated remarkable performance in various medical domains, particularly excelling in tasks that demand confident and precise predictions. These tasks, including Chest-Xray classification,  tumour segmentation, and cardiac catheterization, provide explicit targets at the training time and accordingly expect accurate and certain results in the testing phase.

%Extensive research has confirmed the human-level performance ability of DNNs to identify one or multiple diseases from radiographs 

While DNNs have achieved promising progress, sometimes human-level performance, their translations into real-world clinical decision tools are relatively limited. The reasons are multifactorial. One important gap is between training procedures (discriminating positive and negative labels) and the necessity of communicating uncertainty in health care.

Almost all existing approaches are trained for a determinate binary outcome (either positive or negative) either on image level or pixel level. Their reliance on the standard evaluation metrics, such as accuracy, sensitivity, F1 score, leaves little indication of model abstention when uncertain. 

However, for human physicians, it is natural and routine to communicate uncertainty and ask for a second opinion. For example, in the radiology report, the primary communication means between radiologists and other physicians, there often writes "steaky opacity along the right lung base is \textbf{likely} atelectasis". Uncertainty is an intrinsic aspect of the clinical landscape due to the variability and complexity of medical conditions. Despite the advances of medical knowledge and devices, doctors still face many ambiguous cases in daily work.  The ambiguity and vagueness inherently exist due to the dynamics and complexity of the diseases.  Uncertianty also arises from  scope limitation of medical devices. Imaging modality is only one of important reference for diagnose which is a comprehensive decision. For example, while enlargement of the heart could be observed in Chest X ray, rconfirmation of cardiomegaly needs a blood test or an electrocardiogram.





These uncertain cases pose significant challenges as DNNs may provide overconfident predictions, potentially leading to incorrect diagnoses and harmful conclusions. Unfortunately, this key ability is mainly neglected in existing DNNs. Thus, it is essential to explicitly incorporate the  uncertainty in the framework of DNNs. As called by xxxxx, the model should be able o say "I don't know" and abstain from diagnosing or predicting on uncertain cases. This can boost the reliability of radiology diagnoses, enabling clinicians to make informed decisions, especially in situations where uncertainty is a crucial factor in determining the appropriate course of action for patient care.

% However, almost all of these approaches are only capable of generating a binary outcome (either positive or negative), ignoring the significant aspect of uncertainty in radiology~\pxy{(TODO: make a short review of existing works)}. 



% and some of them have achieved human-level performance~\pxy{(TODO: cite)}.



% Radiology diagnosis, however, differs greatly from those accuracy-oriented tasks. In the domain of radiology diagnosis, uncertain samples are ubiquitous which are neither positive nor negative. This is because uncertainty is an intrinsic aspect of the clinical landscape due to the variability and complexity of medical conditions. \pxy{TODO: give examples here (maybe need example images). Also need to illustrate uncertain causes?} These uncertain cases pose significant challenges as DNNs may provide overconfident predictions, potentially leading to incorrect diagnoses and harmful conclusions. Thus, it is essential to build the capabilities of DNNs to estimate uncertainty and convey confidence levels in their predictions. Incorporating uncertainty estimation in DNNs can boost the reliability of radiology diagnoses, enabling clinicians to make informed decisions, especially in situations where uncertainty is a crucial factor in determining the appropriate course of action for patient care.




In this study, we tackle the important but challenging problem of identifying uncertainty in radiology diagnosis. We developed a novel AI model based on a DNN that is able to distinguish uncertainty from positive and negative. The model is expected to output confident predictions for positive and negative samples but be less confident when it comes to uncertain cases. To this end, we propose to apply a constraint to uncertain samples in training, which punishes the model for being too confident on them. Specifically, this constraint is defined as a target that encourages the model to output a uniform distribution over all the classes. In this case of 2-way classification of positive and negative, the target is to output the same score for the positive and the negative class.

In addition, we also train the model to be noise-robust, as we find it boost the ability of uncertainty identification. In radiograph datasets, label noises usually occur due to mistakes from the automatic labeling tool that extracts labels from medical reports. To tackle the label noise problem, we explore three different noise-robust losses, namely Generalized Cross Entropy (GCE) loss~\cite{}, Partially Huberised Cross Entropy (PCE) loss~\cite{}, and Symmetric Cross Entropy (SCE) loss~\cite{}. Surprisingly, we find that all of the three losses can boost the model's ability to identify uncertainty cases, which is elaborated in Sec.~\ref{}. This demonstrates the adverse effect of noisy labels in radiograph datasets, which has been neglected in most previous works.

% we first recognize that a non-trivial amount of label noise exists in Chest X-ray datasets, which could exert an adverse effect on training. These noisy labels mostly come from the automatic labeling tool that extracts observations from medical reports, while they have been neglected in almost all previous works~\cite{}. Here, we tackle the label noise with a noise-robust loss, which results in a clearer decision boundary than the baseline cross-entropy loss. Then, we propose to explicitly apply a constraint on uncertain samples in training which punishes confident scores on these uncertain cases. Specifically, we use multi-class entropy maximization as the target. In this case of radiology diagnosis, we conduct 2-way classification for positive and negative, so that the entropy maximization target optimizes for a uniform score distribution over the two classes. The overall training target for our model is a combination of the noise-robust loss and the entropy maximization target.

% label noise paper: Improving Medical Image Classification with Label Noise Using Dual-uncertainty Estimation

% uc paper: Learn To Be Uncertain: Leveraging Uncertain Labels In Chest X-rays With Bayesian Neural Networks; 
% Uncertainty-inspired Open Set Learning for Retinal Anomaly Identification


% that the AUC (Area under the ROC Curve) metric, which is adopted by most previous works, is incapable of evaluating uncertainty levels. Thus, we propose to use the Kendall rank correlation coefficient (a.k.a. Kendall's tau) as the metric that counts the number of pairwise agreements and disagreements between two ranking lists. In this case, positive has the highest rank, uncertain is in the middle, and negative is the lowest. In order to achieve a good metric score, positive samples are encouraged to rank higher than uncertain ones and uncertain ones higher than negatives. Then, we find that uncertain samples in most previous works are not adequately leveraged. They are simply ignored in training or roughly mapped to positive or negative samples as a whole. In this work, we propose a novel approach to leveraging uncertain labels via entropy maximization, which penalizes overconfident predictions on uncertain cases. As the proportion of uncertain samples may be very small for some diseases, we also incorporate balanced sampling in the training procedure to emphasize the effect of these uncertain samples.

We conduct extensive experiments on 5 common diseases on two large-scale chest X-ray (CXR) datasets Chexpert and MIMIC-CXR-JPG to validate the effectiveness of our method. It shows that our novel approach to handling uncertainty consistently yields better uncertainty estimations on unseen data than previous approaches. 

The main contributions of this study can be summarised as:

==> sec/intro_v0.tex <==
\section{Introduction}
\label{sec:intro}

Chest X-ray (CXR) is one of the most popular medical imaging technologies in radiology diagnosis\cite{esteva2019guide,litjens2017survey}. These imaging studies play a pivotal role in the assessment of various thoracic conditions, including lung infections, heart abnormalities, and skeletal disorders. Usually, CXR is accompanied by a professional-made medical report of rich information, which comprehensively describes the findings on the patient to facilitate the following intervention or treatment.

Considering the expertise, labor, and extensive time required in manual CXR reading, large-scale CXR datasets have been built to boost the development of artificial intelligence (AI) models for automatic analysis of CXRs~\cite{irvin2019chexpert, johnson2019mimic, johnson2019mimicjpg, wang2017chestx}. Following the longstanding natural image recognition~\cite{krizhevsky2009learning, deng2009imagenet}, these datasets extract from reports category labels for each radiograph, which are typically positive and negative. Such large-scale data with annotations largely supports researchers in developing AI diagnosis models by leveraging the advances in deep learning~\cite{lecun2015deep, he2016deep, krizhevsky2012imagenet}. So far, a number of powerful AI models have been proposed, some of which achieve or even surpass expert-level performance in radiology diagnosis~\cite{yuan2021large, pham2021interpreting}.

% Despite their remarkable performances, a problem with these models is the assumption that the input image for analysis is either positive or negative. This is true with some natural image classification tasks, where an image belongs to either this class or that one~\cite{krizhevsky2009learning, deng2009imagenet}. However, the real-world medical scenario is barely black-and-white. There are many complicated cases of which the analysis is beyond simply positive and negative. For example, Fig.~\ref{fig:moti}(a) shows severe consolidation of a patient, which is a typical positive case. This is in contrast to Fig.~\ref{fig:moti}(b), which is also labeled as positive but is an atypical positive case of a mild symptom. The two cases have a large difference in severity of the disease in spite of their same category labels.

Despite their remarkable performances, a problem with these models is the assumption that the input image for analysis is either positive or negative. This is true with some natural image classification tasks, where the image category is relatively clear~\cite{krizhevsky2009learning, deng2009imagenet}. However, the good man and bad man boundary is not so obvious in medical scenarios.  For example, the report ``there is still very severe bilateral pulmonary consolidation'' of Fig.~\ref{fig:moti}(a) no doubt indicates a typical positive case for consolidation. However, Fig.~\ref{fig:moti}(b) with the description ``substantial
improvement in the right upper lobe consolidation'' shows that the condition of the patient has substantially improved with barely any symptoms left. Though also extracted as positive, the latter is arguably closer to negative in human expert knowledge \pxy{(arguably or considered?)}.

% dazuo:
% Though also extracted as positive, the latter, marked as xxxx colour, should be very close to the decision boundary in Fig xxxxxxx. 


% severe consolidation of a patient, which is a typical positive case. This is in contrast to Fig.~\ref{fig:moti}(b), which is also labeled as positive but is an atypical positive case of a mild symptom. The two cases have a large difference in severity of the disease in spite of their same category labels.


\begin{figure}
    \centering
    \includegraphics[width=\linewidth, trim=7.6cm 1cm 9.6cm 1cm, clip]{figures/hard_6.pdf}
    \caption{Caption}
    \label{fig:hard}
\end{figure}


\begin{figure*}
    \centering
    \includegraphics[width=0.9\textwidth, trim=4cm 6cm 7.3cm 6cm, clip]{figures/moti_a.pdf}
    \includegraphics[width=0.9\textwidth, trim=4cm 6cm 7.3cm 6cm, clip]{figures/moti_b2.pdf}
    \includegraphics[width=0.9\textwidth, trim=4cm 6cm 7.3cm 6cm, clip]{figures/moti_c.pdf}
    \caption{Caption}
    \label{fig:moti}
\end{figure*}

% Ignoring such a disparity within the so-called positive class in cite{????} \pxy{(TODO: cite what?)} can inevitably confuse the classification algorithm. 
Ignoring such a disparity within the so-called positive class in cite{????} \pxy{(TODO: cite what?)} could confuse the classification algorithm. As shown in Fig.~\ref{fig:hard}(a), traditional methods tend to use the Cross Entropy (CE) loss to train a binary classifier~\cite{irvin2019chexpert}. Although training with the CE loss could classify typical negative and positive cases well, predictions on atypical positive cases are likely to be biased. This is because some atypical positive samples with high losses are treated as hard samples. By fitting these hard samples, the model tends to learn an overfitting decision boundary (Fig.~\ref{fig:hard}(b)), resulting in inferior predictions in real-world diagnosis. What is more, this black-and-white separation misses the opportunity to augment medical decision-making with actionable information~\cite{Ehrmann23Npj}. Medical machine learning should be able to say “I’m not sure” when facing ambiguous or uncertainty samples like xxxxxxxxxxx. Knowing when the model is and is not confident in prediction is the fundamental safeguard for safer clinical deployment~\cite{Kompa21Npj}.  

% For example, the atypical case shown in Fig.~\ref{fig:moti}(b) is arguably ``closer'' to a negative case in Fig.~\ref{fig:moti}(c) than to a typical positive case in Fig.~\ref{fig:moti}(a).

% In this way, some atypical positive samples with high losses are treated as hard samples and the model is forced to fit these hard samples. However, fitting these hard samples is likely to result in an overfitting decision boundary, which may not be optimal in real-world radiology diagnosis. due to the fact that some atypical positive cases (\eg, Fig.~\ref{fig:moti}(b)) are ``closer" to negative (\eg, Fig.~\ref{fig:moti}(c)) than to typical positive (\eg, Fig.~\ref{fig:moti}(a)) in human expert evaluation.

% like the one shown in Fig~\ref{fig:moti}(b). In medical practice, however, despite the fact that some atypical positive cases are even "closer" to negative in human expert evaluation.



In this work, we aim to make an AI model learn fine-grained knowledge from medical images so that we can improve the model's ability to diagnose complicated cases that regularly occur in medical practice. To this end, we propose a simple yet effective approach by modulating the risk in the loss function. Specifically, we adopt a new loss function for training, namely the Partially Huberised Cross Entropy (PCE) loss~\cite{feng2021can}, which has a lower risk for hard samples in the low-confidence region. By reducing the risk for hard samples, we can prevent the model from overfitting and expect a decision boundary that is more aligned with human expert evaluation (Fig.~\ref{fig:hard}(c) \& Fig.~\ref{fig:hard}(d)). With such a decision boundary, the model could better communicate fine granularity when faced with complicated clinical cases.

% which enables the model to distinguish atypical and typical positive cases without fine-grained labels.
% adopt a new loss function in training which enables the model to distinguish atypical and typical positive cases without fine-grained labels.
% In this way, we can reduce the model overfitting and expect a decision boundary that is more aligned with human expert evaluation (Fig.~\ref{fig:hard}(c) \& Fig.~\ref{fig:hard}(d)). 

% dazuo:
% We allow the model to communicate uncertainty when faced with an ambiguous clinical case as human physicians.
 
As for evaluation, we first propose a new metric named AUC$^\text{FG}$ for evaluation of fine granularity learning. AUC$^\text{FG}$ calculates the AUC between atypical and typical positive cases of which the criterion is based on a division rule discussed with and validated by human experts. Then, we conduct experiments on the large-scale CXR dataset MIMIC-CXR-JPG~\cite{johnson2019mimicjpg} to validate the proposed method. Experimental results show that, despite its simplicity, our method outperforms baseline approaches by a large margin on two pathologies of clinical significance and prevalence, which demonstrates its effectiveness.

Our main contributions can be summarized as:
\begin{itemize}
    \item We identify the deficiency of learning a simple binary classifier for medical image diagnosis and propose that fine-grained knowledge should be taken into account when building an AI diagnosis system.
    \item We propose a simple yet effective risk modulation approach that allows a model to learn fine granularity from coarsely annotated samples.
    \item We carefully devise a division rule to divide the positive class into atypical positive and typical positive. Based on the division rule, we propose a new metric AUC$^\text{FG}$ for evaluation of fine granularity learning in medical image analysis.
    \item We conduct empirical studies of the proposed method on the large-scale MIMIC-CXR-JPG and demonstrate its superior performance compared with baseline approaches.
\end{itemize}


% p1
% Given that manual radiology diagnosis is time-consuming and 

% p2
% artificial intelligence (AI) models have been developed for the automatic analysis of CXRs~\cite{}. In most cases, these models are trained with coarse categorical labels extracted from CXR reports, which are typically positive and negative~\cite{irvin2019chexpert, wang2017chestx}.

% Considering the expertise, labor, and extensive time required in manual CXR reading, large-scale CXR datasets have been built to boost the development of artificial intelligence (AI) models for automatic analysis of CXRs~\cite{}. To the best of our knowledge, all the publicly available CXR datasets up to now only provide categorical labels at a coarse level, which are typically positive and negative~\cite{}.
% Such a coarse label, however, loses much information in the original rich text content. As shown in Fig.~\ref{fig:moti}, both Fig.~\ref{fig:moti}(a) and Fig.~\ref{fig:moti}(b) are labeled as positive, but a great extinction in severity exists between these two cases. According to the final report, Fig.~\ref{fig:moti}(a) shows severe consolidation of a patient, which is a typical positive case. This is in contrast to Fig.~\ref{fig:moti}(b), which is also labeled as positive but is an atypical positive case of a mild symptom. It is arguable that the atypical positive case shown in Fig.~\ref{fig:moti}(b) is even closer to the negative case in Fig.~\ref{fig:moti}(c) than to the typical positive in Fig.~\ref{fig:moti}(a).


% In the literature, most works utilize the existing coarse labels to train models without considering the medical knowledge. They simply treat the problem as a binary classification, aiming at distinguishing positive and negative cases in the testing time. This leads to a problem that a data point is considered a hard sample when it is not classified correctly in training. Thus, the model is continuously updated to classify the hard samples correctly, even though they may be closer to the opposite class. 

% with the aim of distinguishing positive and negative cases at testing time. Despite the remarkable performances achieved by some state-of-the-art models\cite{}, a significant problem exists that these models do not fully understand the medical knowledge in the data. As shown in Fig.~\ref{fig:moti}, the image in (b) is labeled as positive but is clinically closer to negative. Thus in practice, it is ok for a model to predict a larger negative possibility for such a case. However, if this knowledge is not taken into account in training, the model will simply treat it as a hard sample and be continuously updated to classify it as positive, eliminating the difference between positive samples.

==> sec/method_old.tex <==
\section{Method}
\label{sec:method}

\subsection{Problem Formulation}
We consider a dataset of chest radiographs $X=\{x_i\}^N_{i=1}$ and correspondent labels $Y=\{y_i\}^N_{i=1}$, where $y_i = (y^1_i, y^2_i, ..., y^C_i)$ is a $C$ dimensional vector that contains labels for $C$ observations. In the scenario of radiology diagnosis, the labels for observations are extracted from reports and each observation is assigned to one of positive ($1$), negative ($0$), uncertain ($u$), and blank ($blank$) if it is not mentioned in the report. Label noises usually occur in such a dataset mainly due to ambiguity inherent in the report and mistakes produced by the automatic labeling tool. \pxy{(examples here?)}

Given the medical imaging samples with label noise, our goal in this work is to train a model $f_{\theta}$ with parameters $\theta$ that is capable of identifying uncertain cases in addition to recognizing those explicit positive and negative samples. Although the labels are in the form of multi-label classification~\cite{durand2019learning}, we apply our method to each observation individually in this work. We do this to rule out the potential influence of multi-label learning and thus better focus on the effect of the method itself. Therefore, the output of the model for an observation is $f_{\theta}(x) = (p^n, p^p)$, where $p^n$/$p^p$ represents the probability of being negative/positive. Note that we apply softmax before outputting the probabilities to make sure that $p^n + p^p = 1$. A good uncertainty-aware model should yield $p^n$/$p^p$ close to 1 for negative/positive samples, and $|p^n - p^p|$ close to 0 for uncertain cases. 

\subsection{Uncertainty Learning}
To make a model able to predict uncertainty at testing time, we apply a constraint to uncertain samples in training. In general, the constraint punishes the model for being too confident on uncertain samples, as they are neither explicitly positive nor negative. Specifically, we use a training target that encourages the model to output a uniform distribution over all classes, so that it does not output a high confidence score for any class. In the case of radiology diagnosis, since we conduct a 2-way classification of positive and negative, the target is to output the same score for the positive and the negative class. The target could be written as a loss:
\begin{equation}
    \mathcal{L}_{uc} (y^c=u) = - \frac{1}{2}\log p^n - \frac{1}{2}\log p^p,
\end{equation}
where $c$ is the single observation of interest.
% Note that there are other loss variants that satisfy the goal of the target, such as MSE, MAE, entropy maximization, etc. We choose the cross-entropy loss based on empirical results.

\subsection{Noise-robust Training}
We first deal with the label noise present in the dataset for the purpose of developing a model with better uncertainty identification ability, which is our main goal. The effect of introducing noise-robust training is elaborated in Sec.~\ref{}.

We find that label noises mostly happen to positive or negative samples. On the one hand, there are cases where an interpretation is negative, but the labeler fails to capture the negation meaning and labels it as positive. An example is shown in Figure~\ref{} \pxy{(TODO)}, where the report writes ``\textit{There is resolution of previously seen right middle lobe consolidation.}"
% dicom_id: 11c0c527-512abda9-6682a6ca-3a73bc3a-4d20c153
In clinical usage, ``resolution" refers to past pathological changes improving in the present, with positive findings previously suggesting pathological changes now becoming negative. However, the labeler fails to understand the negative meaning of ``resolution" and produces a positive label for this sample. On the other hand, some cases occur where the labeler falsely takes a positive expression as negative. For example, in this expression ``\textit{There has been no substantial change compared to exam from six hours prior with persistent widespread parenchymal consolidations}'' (Figure.~\ref{}), the labeler simply produces a negative label for consolidation based on ``no'', but the actual description is positive.
% eaa2898d-a7a10f08-33107adb-5f384a51-097283e9

To address this issue, we use the Partially Huberised cross entropy (PCE) loss~\cite{feng2021can} as the training target for positive and negative samples. The PCE loss can be formulated as 
\begin{multline}
    \mathcal{L}_{PCE} (y^c=1) = \\
    \begin{cases}
        % -\tau f(x_i)+\log \tau+1, & \text { if } f(x_i) \leq \frac{1}{\tau} \\
        - \frac{1}{\tau} (p^p - \tau) - \log \tau, & \text{if} \: p^p \leq \tau \\
        -\log p^p, & \text {otherwise}
    \end{cases},
\end{multline}
\begin{multline}
    \mathcal{L}_{PCE} (y^c=0) = \\
    \begin{cases}
        % -\tau f(x_i)+\log \tau+1, & \text { if } f(x_i) \leq \frac{1}{\tau} \\
        - \frac{1}{\tau} (p^n - \tau) - \log \tau, & \text{if} \: p^n \leq \tau \\
        -\log p^n, & \text {otherwise}
    \end{cases},
\end{multline}
where $\tau \in (0, 1)$ is the tangent point of the logarithmic curve. 
% In case the label is $0$, the loss is flipped by $x = 0.5$. 
% The main idea of the robustness of the PCE loss is that the risk of noisy labels is bounded. 
The PCE loss is demonstrated to be noise-robust due to its property of bounded risk in the presence of noisy labels~\cite{}.

\subsection{Training Objective}
The overall training objective incorporates both the uncertainty learning target and the noise-robust loss, which is then written as
\begin{equation}
    \mathcal{L} = \mathcal{L}_{uc} + \lambda \mathcal{L}_{noise},
\end{equation}
where $\mathcal{L}_{noise}$ is either $\mathcal{L}_{PCE}$ or $\mathcal{L}_{GCE}$. We set $\lambda = 1$ throughout this work.

==> sec/method_v0.tex <==
\section{Method}
\label{sec:method}

\subsection{Problem Formulation}
We consider a dataset of chest radiographs $X=\{x_i\}^N_{i=1}$ and correspondent labels $Y=\{y_i\}^N_{i=1}$, where $y_i = (y^1_i, y^2_i, ..., y^C_i)$ is a $C$ dimensional vector that contains labels for $C$ observations. In the scenario of radiology diagnosis, the labels for observations are extracted from reports and each observation is assigned to one of positive ($1$), negative ($0$), uncertain ($u$), and blank ($blank$) if it is not mentioned in the report. 

Given medical images with coarse category labels, our goal in this work is to train a model $f_{\theta}$ with parameters $\theta$ that is capable of communicating fine-grained knowledge in the same class without fine-grained labels. Although the labels are in the form of multi-label classification~\cite{durand2019learning}, we apply our method to each observation individually. We do this to rule out the potential influence of multi-label learning and thus better focus on the effect of the method itself. Therefore, the output of the model for an observation is $f_{\theta}(x) = (p^n, p^p)$, where $p^n$/$p^p$ represents the probability of the sample being negative/positive. Note that we apply softmax before outputting the probabilities to make sure that $p^n + p^p = 1$. 
% A good uncertainty-aware model should yield $p^n$/$p^p$ close to 1 for negative/positive samples, and $|p^n - p^p|$ close to 0 for uncertain cases. 

\subsection{Fine Granularity Learning}
Most previous works simply view radiology diagnosis as a binary classification problem. A common approach is to use the Cross Entropy (CE) loss for training, which is formulated as 
\begin{equation}
    \mathcal{L}_{CE}(y^c) = - (1 - y^c) \log (p^n) - y^c \log (p^p)
\end{equation}
Here, $y^c$ is either $0$ (negative) or $1$ (positive), and we elaborate on how to deal with $y^c = u$ in Sec.~\ref{sec:method_uc}. Although the CE loss can separate easy positive and negative samples, it may not classify borderline cases well due to heavy penalization on hard samples. In radiology diagnosis, however, such a heavy penalization on hard positive samples is not expected, as these hard samples include many atypical positive cases which are arguably closer to negative. Training with the CE loss may lead to model overfitting and misalignment between model perception and human expert evaluation. 

% In this way, all the positive samples are treated in the same manner, but the complexity in real-world medical cases is ignored. Easy positive samples with typical positive patterns tend to have a small loss. However, The CE loss heavily penalizes those hard positive samples with low prediction scores, 

\begin{figure}
    \centering
    \includegraphics[width=\linewidth, trim=0.8cm 0cm 0.7cm 0cm, clip]{figures/curve_CE.pdf}
    \caption{Loss curves for the CE loss and PCE losses with different parameters $\tau$.}
    \label{fig:CE}
\end{figure}

To address this issue, we propose to modulate the risk for hard samples. Specifically, we use the Partially Huberised Cross Entropy (PCE) loss~\cite{feng2021can} as the training target. The PCE loss can be formulated as 
\begin{multline} \label{eq:pce}
    \mathcal{L}_{PCE} (y^c=1) = \\
    \begin{cases}
        % -\tau f(x_i)+\log \tau+1, & \text { if } f(x_i) \leq \frac{1}{\tau} \\
        - \frac{1}{\tau} (p^p - \tau) - \log \tau, & \text{if} \: p^p \leq \tau \\
        -\log p^p, & \text {otherwise}
    \end{cases},
\end{multline}
% \begin{multline}
%     \mathcal{L}_{PCE} (y^c=0) = \\
%     \begin{cases}
%         % -\tau f(x_i)+\log \tau+1, & \text { if } f(x_i) \leq \frac{1}{\tau} \\
%         - \frac{1}{\tau} (p^n - \tau) - \log \tau, & \text{if} \: p^n \leq \tau \\
%         -\log p^n, & \text {otherwise}
%     \end{cases},
% \end{multline}
where $\tau \in (0, 1)$ is the tangent point of the logarithmic curve. As shown in Fig.~\ref{fig:CE}, the PCE loss has a smaller risk and gradient than the CE loss in the low-confidence region (\ie, $\text{x} < \tau$). In this way, we can prevent the model from overfitting and is less likely to overfit hard samples and thus could distinguish atypical and typical cases better. We refer to applying risk modulation on positive samples as P-RM.
% \pxy{(TODO: gradient analysis?)}

The PCE loss was originally proposed to deal with the label noise problem~\cite{feng2021can}. It is demonstrated to be noise-robust due to its property of bounded risk in the presence of noisy labels~\cite{feng2021can}. In this work, we use the same loss function but for a different purpose \pxy{}. We use this risk-bounded loss to show that risk modulation facilitates fine granularity learning within a single class. 


\subsection{Uncertainty Approaches}
\label{sec:method_uc}
Due to the unavoidable ambiguities in medical reports, labels extracted from them could be uncertain (\ie, $y^c = u$) in addition to positive and negative. How to deal with these uncertainty labels varies from work to work and still remains an open problem~\cite{irvin2019chexpert, pham2021interpreting, yuan2021large}. The most common approaches to using uncertainty labels include:
\begin{itemize}
    \item \textbf{Ignoring} (U-Ignore). This approach simply ignores uncertain labels. In multi-label classification, this is achieved by masking losses with respect to samples with uncertainty labels. In this work, as we conduct training for each observation individually, we simply remove samples with uncertainty labels in training for each observation.
    \item \textbf{Binary Mapping}. In this approach, uncertainty labels are all mapped to positive (U-Ones) or all mapped to negative (U-Zeros) as a whole. Compared to U-ignore, this approach takes advantage of the uncertain instances. However, label noises are inevitably introduced in the mapping process, which may mislead the model training and degrade the performance instead~\cite{irvin2019chexpert}.
\end{itemize}

In this work, we propose a new approach termed U-RM to better handling uncertainty labels. We map all uncertainty labels to positive and then apply the risk-modulated loss (\ie, the PCE loss) to them. Similar to fine granularity learning with positive samples, this approach also reduces the punishment on hard uncertain cases that are more likely to be negative. As a result, the model is trained to learn fine granularity from uncertain cases.


\subsection{Training Objective}
The overall training objective incorporates losses on negative, uncertain, and positive samples, which is then written as
\begin{equation}
\begin{split}
    \mathcal{L} = 
     & 1_{[y^c=0]} \cdot \mathcal{L}_{CE}(0) + \\
     & 1_{[y^c=u]} \cdot \mathcal{L}_{PCE}(1) + \\
     & 1_{[y^c=1]} \cdot \mathcal{L}_{PCE}(1)
\end{split}
\end{equation}
Since we apply risk modulation to both positive and uncertain samples, we refer to our method by PU-RM. We set the hyper-parameter $\tau=0.3$ for the PCE loss. Ablation studies on $\tau$ are presented in Sec.~\ref{sec:abl}.




% \subsection{Training Objective}
% The overall training objective incorporates both the uncertainty learning target and the noise-robust loss, which is then written as
% \begin{equation}
%     \mathcal{L} = \mathcal{L}_{uc} + \lambda \mathcal{L}_{noise},
% \end{equation}
% where $\mathcal{L}_{noise}$ is either $\mathcal{L}_{PCE}$ or $\mathcal{L}_{GCE}$. We set $\lambda = 1$ throughout this work.

==> sec_orig/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec_orig/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec_orig/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec_orig/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> tables/atypical.tex <==
\begin{table*}[t]
    \centering
    \begin{tabular}{c|c|c}
        \Xhline{1.5pt}
        & \textbf{Severity} & \textbf{Example Report} \\
        \hline
        \multirow{6}{*}{atypical positive} & trace & \makecell[l]{There is a new \textbf{trace} pleural effusion on the left.} \\
        \cline{2-3}
        & small & \makecell[l]{There is a \textbf{small} right pleural effusion and atelectasis at the right lung base.} \\
        \cline{2-3}
        & tiny & \makecell[l]{There is scattered atelectasis and there are \textbf{tiny} bilateral pleural effusions.} \\
        \cline{2-3}
        & mild & \makecell[l]{There is \textbf{mild} pulmonary vascular congestion and interstitial edema.} \\
        \cline{2-3}
        & minor & \makecell[l]{The right hemithorax segmental atelectasis adjacent to the \textbf{minor} fissure is stable.} \\
        \cline{2-3}
        & minimal & \makecell[l]{Lung volumes are improved with \textbf{minimal} bibasilar atelectasis.} \\
        

        \hline 
        \multirow{3}{*}[-0.7em]{typical positive} & large & \makecell[l]{There is a \textbf{large} heterogeneous consolidation of the right lower lung \\ with air bronchograms compatible with pneumonia.} \\
        \cline{2-3}
        & acute & \makecell[l]{\textbf{Acute} pulmonary congestion with central pulmonary edema \\ and left-sided pleural effusion.} \\
        \cline{2-3} 
        & severe & \makecell[l]{Very \textbf{severe} pulmonary consolidation in the right lung.} \\


        \Xhline{1.5pt}
        % \multicolumn{3}{c}{\textbf{(b) Change in time}} \\
        & \textbf{Change in time} & \textbf{Example Report} \\
        
        \hline
        \multirow{4}{*}[-1.8em]{atypical positive} & clear & \makecell[l]{Since \underline{\hspace{0.5cm}}, the volume of consolidation in the right mid and \\ lower lung zone has decreased and pulmonary edema has largely \textbf{clear}ed.} \\
        \cline{2-3}
        & resolution & \makecell[l]{Cardiomegaly is accompanied by improved pulmonary vascular congestion \\ and near \textbf{resolution} of interstitial edema. } \\
        \cline{2-3}
        & improve & \makecell[l]{The left hemidiaphragm and left costophrenic sulcus are now better defined, \\ 
        suggesting interval \textbf{improvement} in the left lower lobe collapse/consolidation.} \\
        \cline{2-3}
        & decrease & \makecell[l]{As compared to the previous radiograph, the signs of interstitial lung edema \\ have \textbf{decrease}d in extent and severity.} \\

        \hline
        \multirow{3}{*}[-0.7em]{typical positive} & progress & \makecell[l]{There is interval \textbf{progress}ion of vascular congestion and interstitial pulmonary edema.} \\
        \cline{2-3}
        & worsen & \makecell[l]{Moderate to severe pulmonary edema has \textbf{worsen}ed.} \\
        \cline{2-3} 
        & increase & \makecell[l]{Since the chest radiographs obtained 3 days prior, there has been \\ a significant \textbf{increase} in left lung atelectasis with leftward mediastinal shift.} \\
        
        \Xhline{1.5pt}
    \end{tabular}
    \caption{Caption}
    \label{tab:atypical}
\end{table*}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{c|c|c}
%         \toprule
%         & Severity & Change in time \\
%         \midrule
%         \makecell[l]{atypical \\ positive} & \makecell[l]{trace \\ mild \\ minor \\ subtle \\ minimal \\ small \\ mild-to-moderate} & \makecell[l]{clear \\ resolution \\ improve \\ decrease} \\
%         \midrule
%         \makecell[l]{typical \\ positive} & \makecell[l]{moderate \\ moderate-to-severe \\ massive \\ acute \\ severe} & \makecell[l]{progress \\ worsen \\ increase} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:atypical}
% \end{table}

% \begin{table}[t]
%     \centering
%     \begin{tabular}{c|c|c}
%         \toprule
%         & Severity & Change in time \\
%         \midrule
%         \makecell[l]{atypical \\ positive} & \makecell[l]{\textit{mild} \\ \textit{minor} \\ \textit{subtle} \\ \textit{minimal} \\ \textit{small} \\ \textit{mild-to-moderate}} & \makecell[l]{\textit{clear} \\ \textit{resolution} \\ \textit{improve} \\ \textit{decrease}} \\
%         \midrule
%         \makecell[l]{typical \\ positive} & \makecell[l]{\textit{moderate} \\ \textit{moderate-to-severe} \\ \textit{massive} \\ \textit{acute} \\ \textit{severe}} & \makecell[l]{\textit{progress} \\ \textit{worsen} \\ \textit{increase}} \\
%         \bottomrule
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:atypical}
% \end{table}


==> tables/atypical3.tex <==
\begin{table*}[t]
    \centering
    \begin{subtable}[h]{\linewidth}
    \begin{tabular}{c|c|c}
        \toprule
        & \makecell{Fine \\ Text-Mined Label} & Example Report \\
        \midrule
        \multirow{6}{*}[-1.6em]{\makecell{atypical \\ positive}} & trace & \makecell[l]{There is a new \textbf{trace} pleural effusion on the left.} \\
        \cline{2-3}
        & small & \makecell[l]{There is a \textbf{small} right pleural effusion and atelectasis at the right lung base.} \\
        \cline{2-3}
        & tiny & \makecell[l]{There is scattered atelectasis and there are \textbf{tiny} bilateral pleural effusions.} \\
        \cline{2-3}
        & minor & \makecell[l]{The right hemithorax segmental atelectasis adjacent to the \textbf{minor} fissure \\ is stable.} \\
        \cline{2-3}
        & minimal & \makecell[l]{Lung volumes are improved with \textbf{minimal} bibasilar atelectasis.} \\
        \cline{2-3}
        & mild & \makecell[l]{There is \textbf{mild} pulmonary vascular congestion and interstitial edema.} \\
        \cline{2-3}
        & mild-to-moderate & \makecell[l]{In comparison with the study of \underline{\hspace{0.5cm}}, there is continued substantial \\ cardiomegaly with \textbf{mild-to-moderate} pulmonary edema.} \\
        
        \hline 
        \multirow{4}{*}[-4.2em]{\makecell{typical \\ positive}} & large & \makecell[l]{There is a \textbf{large} heterogeneous consolidation of the right lower lung with \\ air bronchograms compatible with pneumonia.} \\
        \cline{2-3}
        & massive & \makecell[l]{Frontal and lateral radiographs of the chest demonstrate persistent \textbf{massive} \\ left-sided pleural effusion, occupying at least two-thirds of the left hemithorax.} \\
        \cline{2-3}
        & substantial & \makecell[l]{Diffuse bilateral pulmonary opacifications are again seen, consistent with \\ \textbf{substantial} pulmonary edema.} \\
        \cline{2-3}
        & moderate & \makecell[l]{There continues to be a moderate left effusion.} \\
        \cline{2-3}
        & moderate-to-severe & \makecell[l]{There is interval development of \textbf{moderate-to-severe} interstitial pulmonary \\ edema with some element of alveolar edema and bilateral pleural effusions,} \\
        \cline{2-3}
        & acute & \makecell[l]{\textbf{Acute} pulmonary congestion with central pulmonary edema and left-sided \\ pleural effusion.} \\
        \cline{2-3} 
        & severe & \makecell[l]{Very \textbf{severe} pulmonary consolidation is seen in the right lung.} \\
        
        \bottomrule
    \end{tabular}
    \caption{Division based on severity.}
    \label{tab:div_svr}
    \end{subtable}
    
    % \vspace{1em}
    \begin{subtable}[h]{\linewidth}
    \begin{tabular}{c|c|c}
        \toprule
        & \makecell{Fine \\ Text-Mined Label} & Example Report \\
        
        \midrule
        \multirow{4}{*}[-1.8em]{\makecell{atypical \\ positive}} & clear & \makecell[l]{Since \underline{\hspace{0.5cm}}, the volume of consolidation in the right mid and \\ lower lung zone has decreased and pulmonary edema has largely \textbf{clear}ed.} \\
        \cline{2-3}
        & resolution & \makecell[l]{Cardiomegaly is accompanied by improved pulmonary vascular congestion \\ and near \textbf{resolution} of interstitial edema. } \\
        \cline{2-3}
        & improve & \makecell[l]{The left hemidiaphragm and left costophrenic sulcus are now better defined, \\ 
        suggesting interval \textbf{improvement} in the left lower lobe collapse/consolidation.} \\
        \cline{2-3}
        & decrease & \makecell[l]{As compared to the previous radiograph, the signs of interstitial lung edema \\ have \textbf{decrease}d in extent and severity.} \\

        \hline
        \multirow{3}{*}[-0.7em]{\makecell{typical \\ positive}} & progress & \makecell[l]{There is interval \textbf{progress}ion of vascular congestion and interstitial \\ pulmonary edema.} \\
        \cline{2-3}
        & worsen & \makecell[l]{Moderate to severe pulmonary edema has \textbf{worsen}ed.} \\
        \cline{2-3} 
        & increase & \makecell[l]{Since the chest radiographs obtained 3 days prior, there has been \\ a significant \textbf{increase} in left lung atelectasis with leftward mediastinal shift.} \\
        
        \bottomrule
    \end{tabular}
    \caption{Division based on change in time.}
    \label{tab:div_change}
    \end{subtable}
    \caption{Caption}
    \label{tab:fg_div}
\end{table*}

==> tables/main_res_old.tex <==
% \usepackage{makecell}

\begin{table}[t]
\centering
\small
% \addtolength{\tabcolsep}{-5.pt}
\begin{tabular}{c|cccc}

\Xhline{1.0pt}
% \toprule
\multicolumn{5}{c}{\textbf{(a) Consolidation}} \\
Method\textbackslash Metric & AUC$_{p/n}$ & AUC$_{p/uc}$ & AUC$_{uc/n}$ & AUC$_{mean}$ \\
\hline
UC-Ignore & 0.9464 & 0.6917 & 0.8536 & 0.8302 \\
UC-Zeros & 0.9468 & \textbf{0.7019} & 0.8577 & \textbf{0.8354} \\
UC-Ones & 0.9495 & 0.6834 & \textbf{0.8660} & 0.8330 \\
Ours (PCE) & 0.9465 & 0.6936 & \textbf{0.8659} & \textbf{0.8353} \\
Ours (GCE) & 0.9457 & 0.6949 & 0.8634 & 0.8347 \\


\Xhline{1.0pt}
\multicolumn{5}{c}{\textbf{(b) Edema}}  \\
Method\textbackslash Metric & AUC$_{p/n}$ & AUC$_{p/uc}$ & AUC$_{uc/n}$ & AUC$_{mean}$ \\
\hline
UC-Ignore & 0.9171 & 0.5013 & 0.9066 & 0.7750  \\
UC-Zeros & 0.9140 & 0.5608 & 0.8892 & 0.7880  \\
UC-Ones & 0.9192 & 0.4881 & 0.9114 & 0.7729  \\
Ours (PCE) & 0.9164 & 0.5424 & 0.9039 & 0.7876  \\
Ours (GCE) & 0.9156 & 0.5608 & 0.8992 & 0.7919  \\


\Xhline{1.0pt}
\multicolumn{5}{c}{\textbf{(c) Pleural Effusion}}  \\
Method\textbackslash Metric & AUC$_{p/n}$ & AUC$_{p/uc}$ & AUC$_{uc/n}$ & AUC$_{mean}$ \\
\hline
UC-Ignore & 0. & 0. & 0. & 0.  \\
UC-Zeros & 0. & 0. & 0. & 0.  \\
UC-Ones & 0. & 0. & 0. & 0.  \\
Ours (PCE) & 0. & 0. & 0. & 0.  \\
Ours (GCE) & 0. & 0. & 0. & 0.  \\


\Xhline{1.0pt}
% \bottomrule
\end{tabular}
\normalsize
\caption{Caption.}
\label{tab:main_res}
\end{table}
